Neural Network Branch-and-Bound for Neural Network Verification

Many available formal verification methods have been shown to be instances of a unified Branch-and-Bound (BaB) formulation. We propose a novel machine learning framework that can be used for designing an effective branching strategy as well as for computing better lower bounds. Specifically, we learn two graph neural networks (GNN) that both directly treat the network we want to verify as a graph input and perform forward-backward passes through the GNN layers. We use one GNN to simulate the strong branching heuristic behaviour and another to compute a feasible dual solution of the convex relaxation, thereby providing a valid lower bound. We provide a new verification dataset that is more challenging than those used in the literature, thereby providing an effective alternative for testing algorithmic improvements for verification. Whilst using just one of the GNNs leads to a reduction in verification time, we get optimal performance when combining the two GNN approaches. Our combined framework achieves a 50\% reduction in both the number of branches and the time required for verification on various convolutional networks when compared to several state-of-the-art verification methods. In addition, we show that our GNN models generalize well to harder properties on larger unseen networks.

==> Algorithms/BaB_Jodie.tex <==
\begin{algorithm}[H]
                  \caption{Branch and Bound}\label{alg:bab}
                  \small 
                  \begin{algorithmic}[1]
                    \algrenewcommand\algorithmicindent{1.0em}%
                    \Function{BaB}{$\mtt{net}, \mtt{problem}, \epsilon$}
                    \State $\mtt{global\_lb} \gets {\mtt{compute\_LB}}(\mtt{net}, \mtt{problem})$
                    \State $\mtt{global\_ub} \gets {\mtt{compute\_UB}}(\mtt{net}, \mtt{problem})$
                    \State $\mtt{probs}\gets \left[ (\mtt{global\_lb}, \mtt{problem}) \right]$
                    \While{$\mtt{global\_ub} - \mtt{global\_lb} > \epsilon $}
                    \State $(\_\ , \mtt{prob}) \gets \mtt{pick\_out}(\mtt{probs})$
                    \State $\left[ \mtt{subprob\_1}, \dots, \mtt{subprob\_s} \right] \gets \mtt{split}(\mtt{prob})$
                    \For{$i = 1 \dots s $}
                    \State $\mtt{sub\_lb} \gets {\mtt{compute\_LB}}(\mtt{net}, \mtt{subprob\_i})$
                    \State $\mtt{sub\_ub} \gets \mtt{compute\_UB}(\mtt{net}, \mtt{subprob\_i})$
                    \If{$\mtt{sub\_ub} < \mtt{global\_ub}$}
                    \State $\mtt{global\_ub} \gets \mtt{sub\_ub}$
                    \State $\mtt{prune\_probs}(\mtt{probs}, \mtt{global\_ub})$
                    \EndIf
                    \If{$\mtt{sub\_lb} < \mtt{global\_ub}$}
                    \State $\mtt{probs}.\mtt{append}((\mtt{sub\_lb}, \mtt{subprob\_i}))$
                    \EndIf
                    \EndFor
                    \State $\mtt{global\_lb} \gets \min\{ \mtt{lb}\ |\ (\mtt{lb}, \mtt{prob}) \in \mtt{probs}\}$
                    \EndWhile
                    \State\Return $\mtt{global\_ub}$
                    \EndFunction
                  \end{algorithmic}
\end{algorithm}

==> Algorithms/Generating_Training_Dataset.tex <==
\begin{algorithm}[H]
  \caption{Generating Training Dataset}\label{alg:train-gen}
  \begin{algorithmic}[1]
    \State{Provided: total $P$ properties; minimum $B$ training data for each property; a maximum $q$ branches between strong branching decisions}
    \For{$p = 1, \dots, P$}:
     \State{$\alpha \longleftarrow \text{random number from }[0, 1]$}
     \If{$p$ is not a timed out property and $\alpha \leq 0.25$ }
        \State{Running a complete BaB process with the Strong Branching Heuristic}
     \Else
        \State{$b=0$}
        \While{$b\leq B$}    
             \State{$k \longleftarrow \text{random integer from} [0, q]$}
             \While{$k >0$}
                \State{Call a computationally cheap heuristic}
             \If{BaB process terminates}
                 \Return
             \EndIf
             \State{$k = k -1 $}
        \EndWhile
        \State{Call the strong branching heuristic and generate a training sample}
        \If{BaB process terminates}
             \Return
        \EndIf
        \State{$b=b+1$}
    \EndWhile
    \EndIf
    \EndFor
  \end{algorithmic}
\end{algorithm}

==> Tables/branching_base_model.tex <==
\sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table}[t]
\vspace{-10pt}
\centering
\caption{\footnotesize Methods' Performance on the Base model. For easy, medium and difficult level verification properties, we compare methods' average solving time, average number of branches required and the percentage of timed out properties. GNN-Branching outperforms other methods in all aspects (Note that by definition Gurobi BaBSR doesn't time out on easy and med experiments).}
\label{table:base-model}
\vspace{-8pt}
\scriptsize
\setlength{\tabcolsep}{4pt}
\aboverulesep = 0.1mm  % 0.605mm
\belowrulesep = 0.2mm  % 0.984mm
\begin{adjustbox}{center}
\begin{tabular}{
    l
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    }
    & \multicolumn{3}{ c }{Easy} & \multicolumn{3}{ c }{Medium} & \multicolumn{3}{ c }{Hard} \\
    \toprule

    \multicolumn{1}{ c }{Method} &
    \multicolumn{1}{ c }{time(s)} &
    \multicolumn{1}{ c }{branches} &
    \multicolumn{1}{ c }{$\%$Timeout} &
    \multicolumn{1}{ c }{time(s)} &
    \multicolumn{1}{ c }{branches} &
    \multicolumn{1}{ c }{$\%$Timeout} &
    \multicolumn{1}{ c }{time(s)} &
    \multicolumn{1}{ c }{branches} &
    \multicolumn{1}{ c }{$\%$Timeout} \\

    \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}

    \multicolumn{1}{ c }{\textsc{BaBSR}}
        &545.457
        &578.828
        &0.0

        &1370.395
        &1405.301
        &0.0

        &3127.995
        &2493.870
        &41.3 \\

    \multicolumn{1}{ c }{\textsc{MIPplanet}}
        &1499.375
        & 
        &16.5

        &2240.980
        & 
        &43.0

        &2250.623
        & 
        &46.2 \\

    \multicolumn{1}{ c }{\textsc{GNN-branching}}
        &\B272.695
        &\B285.682
        &\B0.2

        &\B592.118
        &\B583.210
        &\B0.4

        &\B1577.156
        &\B995.437
        &\B21.6 \\

    % \multicolumn{1}{ c }{\textsc{GNN-online}}
    %      &\B 208.821
    %      &\B 252.807
    %      &\B 0.002

    %      &\B 556.163
    %      &\B 501.595
    %      &\B 0.001

    %      &\B 1369.326
    %      &\B 813.502
    %      &\B 0.183 \\

    \bottomrule

\end{tabular}
\end{adjustbox}
\vspace{-10pt}
\end{table}

==> Tables/branching_large_models.tex <==
\sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table}[h]
\centering
% \footnotesize
\caption{\footnotesize Methods' Performance on Large Models. For verification properties on Wide large model and Deep large model, we compare methods' average solving time, average number of branches required and the percentage of timed out properties. We use a timeout of 7200s. GNN-branching outperforms bother baselines in all aspects.}
\label{table:large-models}
\vspace{-10pt}
\scriptsize
\setlength{\tabcolsep}{4pt}
\aboverulesep = 0.1mm  % 0.605mm
\belowrulesep = 0.2mm  % 0.984mm
\begin{tabular}{
    l
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    S[table-format=4.3]
    }
    & \multicolumn{3}{ c }{Wide} & \multicolumn{3}{ c }{Deep} \\
    \toprule

    \multicolumn{1}{ c }{Method} &
    \multicolumn{1}{ c }{time} &
    \multicolumn{1}{ c }{branches} &
    \multicolumn{1}{ c }{$\%$Timeout} &
    \multicolumn{1}{ c }{time} &
    \multicolumn{1}{ c }{branches} &
    \multicolumn{1}{ c }{$\%$Timeout} \\

    \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} 

    \multicolumn{1}{ c }{\textsc{BaBSR}}
        &4137.467
        &843.476
        &??

        &4016.336
        &416.824
        &?? \\

    \multicolumn{1}{ c }{\textsc{MIPplanet}}
        &5855.059
        & 
        &74.3

        &5426.160
        & 
        &60.8 \\

    \multicolumn{1}{ c }{\textsc{GNN-branching}}
        &\B 2367.693
        &\B 387.403
        &\B 12.7

        &\B 2308.612
        &\B 208.760
        &\B 4.8 \\

    % \multicolumn{1}{ c }{\textsc{GNN-online}}
    %      &\B 2179.306
    %      &\B 353.879
    %      &\B 0.095

    %      &\B 2220.351
    %      &\B 199.032
    %      &\B 0.040 \\

    \bottomrule

\end{tabular}

\end{table}

==> Tables/head_to_head.tex <==

% \subsection{Tables in process}
 \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
%\begin{table*}[t!]
\begin{table*}[h]
	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}

	\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			} \\
			& \multicolumn{4}{ c }{Base} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}} &
			\multicolumn{1}{ c }{\textsc{MIPplanet}} &
			\multicolumn{1}{ c }{\textsc{Supergradient}} &
			\multicolumn{1}{ c }{\textsc{GNN im 20}} &
			\multicolumn{1}{ c }{Best} & \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-6}
			
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}}
			&
            & \B 60.44
            & 0.77
            & 0.70
			
			&0.07\\
			
			\multicolumn{1}{ c }{\textsc{MIPplanet}}
             & 39.56
             &
             & 18.10
             & 17.96
    			
			 &17.96 \\
			
			\multicolumn{1}{ c }{\textsc{Supergradient}}
             & \B 99.23
             & \B 81.90
             &
             & 6.95
			
			 &4.05\\
			
			\multicolumn{1}{ c }{\textsc{GNN}}
             & \B 99.30
             & \B 82.04
             & \B 93.05
			 &
			
			 & \B 77.92 \\
			\bottomrule
			
		\end{tabular}
		\end{adjustbox}


		\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			} \\
			& \multicolumn{4}{ c }{Wide} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}} &
			\multicolumn{1}{ c }{\textsc{MIPplanet}} &
			\multicolumn{1}{ c }{\textsc{Supergradient}} &
			\multicolumn{1}{ c }{\textsc{GNN im 100}} &
			\multicolumn{1}{ c }{Best} & \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-6}
			
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}}
			&
			&\B 71.67
			&1.61
			&1.61
			
			&0.37\\
			
			\multicolumn{1}{ c }{\textsc{MIPplanet}}
			&28.33
			&
			&13.81
			&14.23
			
			&13.43 \\
			
			\multicolumn{1}{ c }{\textsc{Supergradient}}
			&\B 98.39
			&\B 86.19
			&
			&14.57
			
			&12.31\\
			
			\multicolumn{1}{ c }{\textsc{GNN}}
			&\B 98.39
			&\B 85.77
			&\B 85.43
			&
			
			&\B 73.88 \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	
	
	\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			} \\
			& \multicolumn{4}{ c }{Deep} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}} &
			\multicolumn{1}{ c }{\textsc{MIPplanet}} &
			\multicolumn{1}{ c }{\textsc{Supergradient}} &
			\multicolumn{1}{ c }{\textsc{GNN im 100}} &
			\multicolumn{1}{ c }{Best} & \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-6}
			
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}}
			&
			& \B 61.97
			&1.29
			&1.28
			
			&0.41\\
			
			\multicolumn{1}{ c }{\textsc{MIPplanet}}
			&38.03
			&
			&9.21
			&8.71
			
			&8.26 \\
			
			\multicolumn{1}{ c }{\textsc{Supergradient}}
			& \B 98.71
			& \B 90.79
			&
			&25.86
			
			&22.73\\
			
			\multicolumn{1}{ c }{\textsc{GNN}}
			& \B 98.72
			& \B 91.29
			& \B 74.14
			&
			
			& \B 68.60 \\
			\bottomrule
			
		\end{tabular}

		
	\end{adjustbox}
	
	
	\caption{\small We compare head-to-head performance of the different methods on the base, wide, and deep model. The numbers refer to the percentage of images on which the method in the row header beats the method in the column header. The final column represents the percentage of images on which the method beats all other methods. If two models timeout on an image than that image is not included in their head-to-head performance as neither method beats the other. The better performing method is highlighted in bold}
	\label{table:head_to_head}
\end{table*}

==> Tables/network_architecture.tex <==
\begin{table}[h!]
	\centering
	\small
	\begin{tabular}{|c|c|c|}
		\hline
		\textbf{Network Name}\TBstrut & \textbf{No. of Properties} \TBstrut & \textbf{Network Architecture} \TBstrut\\
		\hline
		\begin{tabular}{l}
			BASE \\ 
			Model
		\end{tabular} & \begin{tabular}{@{}c@{}}
		    Training: 430  \\
			Easy: 425 (\citet{lu2019neural}: 467)  \\
			Medium: 704 (\citet{lu2019neural}: 773) \\
			Hard: 387 (\citet{lu2019neural}: 426)
		\end{tabular} & \begin{tabular}{@{}c@{}} 
			\footnotesize
			Conv2d(3,8,4, stride=2, padding=1) \Tstrut \\
			Conv2d(8,16,4, stride=2, padding=1)\\
			linear layer of 100 hidden units \\
			linear layer of 10 hidden units\\
			(Total ReLU activation units: 3172) \Bstrut
		\end{tabular}\\
		\hline
		WIDE & 300 & \begin{tabular}{@{}c@{}} 
			\footnotesize
			Conv2d(3,16,4, stride=2, padding=1) \Tstrut\\
			Conv2d(16,32,4, stride=2, padding=1)\\
			linear layer of 100 hidden units \\
			linear layer of 10 hidden units\\
			(Total ReLU activation units: 6244) \Bstrut
		\end{tabular}\\
		\hline
		DEEP & 250 & \begin{tabular}{@{}c@{}} 
			\footnotesize
			Conv2d(3,8,4, stride=2, padding=1) \Tstrut \\
			Conv2d(8,8,3, stride=1, padding=1) \\
			Conv2d(8,8,3, stride=1, padding=1) \\
			Conv2d(8,8,4, stride=2, padding=1)\\
			linear layer of 100 hidden units \\
			linear layer of 10 hidden units\\
			(Total ReLU activation units: 6756) \Bstrut
		\end{tabular}\\
		\hline
	\end{tabular}
	\caption{\label{tab:problem_size} Network Architectures}%For each complete verification experiment, the network architecture used and the number of verification properties tested, from the dataset by \citet{lu2019neural}. Each layer but the last is followed by a ReLU activation function. For some of the property classes, we employed only a subset of the original data due to computational constraints.}
\end{table}

==> Tables/table_all.tex <==

% \subsection{Tables in process}
 \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
\begin{table*}[t]
	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}
    
	\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			}
			& \multicolumn{3}{ c }{Base} & \multicolumn{3}{ c }{Wide} & \multicolumn{3}{ c }{Deep} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
			
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}}
			&1588.02
			&1340.08
			&10.57
			
			&2917.95
			&855.37
			&51.11
			
			&3007.24
			&428.52
			&54.00 \\
			
			\multicolumn{1}{ c }{\textsc{MIPplanet}}
			& 2036.65
			& 
			&36.40
			
			& 3108.50
			& 
			&79.37
			
			& 2997.12
			& 
			&73.60 \\
			
			\multicolumn{1}{ c }{\textsc{Supergradient}}
			&293.10
			&8165.67
			&4.68
			
			& 644.93
			& 8287.48
			& 13.20
			
			&277.44
			&3314.22
			&4.00 \\
			
			\multicolumn{1}{ c }{\textsc{GNN-branching}}
			& 752.94
			& 604.16
			& 5.77
			
			& 1817.97
			& 418.68
			& 21.27
			
			& 1966.90
			& 202.73
			& 20.80\\

			\multicolumn{1}{ c }{\textsc{GNN-bounding}}
			& 219.62
			& 6427.10
			& 2.94
			
			& 513.63
			& 5274.19
			& 10.23
			
			& 214.55
			& 2784.49
			& 2.80\\

			\multicolumn{1}{ c }{\textsc{GNN-combined}}
			&\B 143.04
			& 3556.60
			&\B 1.44
			
			&\B 305.42
			& 2867.50
			&\B 5.61
			
			&\B 111.74
			& 1512.52
			&\B 0.80\\

			\bottomrule
			
		\end{tabular}
	\end{adjustbox}
	\caption{\small We compare average (mean) solving time, average number of subdomains solved, and the percentage of properties that the methods time out on when using a cut-off time of 3600s. The best performing method for each subcategory is highlighted in bold.}
	\label{table:combined_base_wide_deep}
\end{table*}

==> Tables/table_all_base.tex <==

% \subsection{Tables in process}
 \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
%\begin{table*}[t!]
\begin{table*}[t]
	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}

	\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			}
			& \multicolumn{3}{ c }{Easy} & \multicolumn{3}{ c }{Med} & \multicolumn{3}{ c }{Hard} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
			
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}}
			&550.48
			&580.43
			&0.00
			
			&1374.32
			&1408.75
			&0.00
			
			&3129.08
			&2551.63
			&42.41 \\
			
			\multicolumn{1}{ c }{\textsc{MIPplanet}}
			&1499.35
			& 
			&16.49
			
			&2240.92
			& 
			&42.95

			&2255.53
			& 
			&46.35 \\
			
			\multicolumn{1}{ c }{\textsc{Supergradient}}
			&59.40
			&2528.48
			&0.21
			
			&87.71
			&5289.22
			&\B0.00
			
			&923.45
			&22103.66
			&18.12 \\
			
			\multicolumn{1}{ c }{\textsc{GNN_Branching}}
			&272.69
			&285.68
			&0.21
			
			&592.12
			&583.21
			& 0.39
			
			&1573.16
			&1098.28
			&21.65 \\

			\multicolumn{1}{ c }{\textsc{GNN_Bounding}}
			&\B46.70
			&2201.70
			&\B0.00
			
			&78.85
			&4108.27
			&\B 0.00
			
			&665.64
			&16442.30
			&11.53 \\

			\multicolumn{1}{ c }{\textsc{GNN_Combined}}
			&50.61
			&1188.36
			&0.21
			
			&\B68.52
			&2419.44
			&\B 0.00
			
			&\B380.15
			&8488.50
			&\B5.41 \\

			\bottomrule
			
		\end{tabular}
	\end{adjustbox}
	\caption{\small We compare average (mean) solving time, average number of subdomains solved, and the percentage of properties solved for easy, medium, and hard properties on the base model. The best performing method for each subcategory is highlighted in bold (note that by definition Gurobi BaBSR doesn't time out on easy and med experiments).}.
	\label{table:combined_base_exp}
\end{table*}

==> Tables/table_all_base__h_.tex <==

% \subsection{Tables in process}
 \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
%\begin{table*}[t!]
\begin{table*}[h]
	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}

	\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			}
			& \multicolumn{3}{ c }{Easy} & \multicolumn{3}{ c }{Med} & \multicolumn{3}{ c }{Hard} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
			
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}}
			&550.48
			&580.43
			&0.00
			
			&1374.32
			&1408.75
			&0.00
			
			&3129.08
			&2551.63
			&42.41 \\
			
			\multicolumn{1}{ c }{\textsc{MIPplanet}}
			&1499.35
			& 
			&16.49
			
			&2240.92
			& 
			&42.95

			&2255.53
			& 
			&46.35 \\
			
			\multicolumn{1}{ c }{\textsc{Supergradient}}
			&59.40
			&2528.48
			&0.21
			
			&87.71
			&5289.22
			&\B0.00
			
			&923.45
			&22103.66
			&18.12 \\
			
			\multicolumn{1}{ c }{\textsc{GNN_Branching}}
			&272.69
			&285.68
			&0.21
			
			&592.12
			&583.21
			& 0.39
			
			&1573.16
			&1098.28
			&21.65 \\

			\multicolumn{1}{ c }{\textsc{GNN_Bounding}}
			&\B46.70
			&2201.70
			&\B0.00
			
			&78.85
			&4108.27
			&\B 0.00
			
			&665.64
			&16442.30
			&11.53 \\

			\multicolumn{1}{ c }{\textsc{GNN_Combined}}
			&50.61
			&1188.36
			&0.21
			
			&\B68.52
			&2419.44
			&\B 0.00
			
			&\B380.15
			&8488.50
			&\B5.41 \\

			\bottomrule
			
		\end{tabular}
	\end{adjustbox}
	\caption{\small We compare average (mean) solving time, average number of subdomains solved, and the percentage of properties solved for easy, medium, and hard properties on the base model. The best performing method for each subcategory is highlighted in bold (note that by definition Gurobi BaBSR doesn't time out on easy and med experiments).}.
	\label{table:combined_base_exp[h]}
\end{table*}

==> Tables/table_base_median.tex <==

% \subsection{Tables in process}
 \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
%\begin{table*}[t!]
\begin{table*}[h]
	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}

	\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			}
			& \multicolumn{3}{ c }{Easy} & \multicolumn{3}{ c }{Med} & \multicolumn{3}{ c }{Hard} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
			
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}}
			&471.547
			&468.117
			&0.0
			
			&1304.032
			&1236.398
			&0.0
			
			&3094.794
			&2271.796
			&0.413 \\
			
			\multicolumn{1}{ c }{\textsc{MIPplanet}}
			&836.049
			& 
			&0.165
			
			&1401.273
			& 
			&0.430
			
			&1374.794
			& 
			&0.462 \\
			
			\multicolumn{1}{ c }{\textsc{Supergradient}}
			&81.069
			&2347.969
			&0.002
			
			&165.769
			&5594.891
			&0.002
			
			&282.139
			&9961.521
			&0.003 \\
			
			\multicolumn{1}{ c }{\textsc{GNN im 20}}
			&73.136
			&2103.566
			&0.002
			
			& 159.073
			& 5313.910
			& 0.002
			
			& 289.592
			& 10032.108
			& 0.003 \\
			
			\multicolumn{1}{ c }{\textsc{GNN50}}
			& \B 65.760
			& \B 1848.276
			& 0.002
			
			& \B 146.250
			& \B 4858.806
			& 0.002
			
			& \B 259.33
			& \B 9064.482
			& 0.003 \\
			
			\multicolumn{1}{ c }{\textsc{GNN100}}
			&69.297
			&1982.463
			&0.002
			
			& 152.651
			& 5092.674
			& 0.002
			
			& 269.625
			& 9436.066
			& 0.003 \\
		
			\bottomrule
			
		\end{tabular}
	\end{adjustbox}
	\caption{\small We compare average(median) solving time, average(median) number of subdomains solved, and the percentage of properties solved for easy, medium, and hard properties on the base model. The best performing method for each subcategory is highlighted in bold. (Note that by definition Gurobi BaBSR doesn't time out on easy and med experiments)}
	\label{table:easy_med_hard}
\end{table*}

==> Tables/table_easy_med_hard.tex <==

% \subsection{Tables in process}
 \sisetup{detect-weight=true,detect-inline-weight=math,detect-mode=true}
%\begin{table*}[t!]
\begin{table*}[h]
	\centering
	\scriptsize
	\setlength{\tabcolsep}{4pt}
	\aboverulesep = 0.1mm  % 0.605mm
	\belowrulesep = 0.2mm  % 0.984mm
	
	% bold elements in table
	%\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    %\renewrobustcmd{\boldmath}{}
    %\newrobustcmd{\B}{\bfseries}

	\begin{adjustbox}{center}
		\begin{tabular}{
				l
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
				S[table-format=4.3]
			}
			& \multicolumn{3}{ c }{Easy} & \multicolumn{3}{ c }{Med} & \multicolumn{3}{ c }{Hard} \\
			\toprule
			
			\multicolumn{1}{ c }{Method} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} &
			\multicolumn{1}{ c }{time(s)} &
			\multicolumn{1}{ c }{subdomains} &
			\multicolumn{1}{ c }{$\%$Timeout} \\
			
			\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
			
			\multicolumn{1}{ c }{\textsc{Gurobi BaBSR}}
			&550.48
			&\B584.53
			&\B0.00
			
			&1374.32
			&\B1411.19
			&\B0.00
			
			&3132.97
			&\B2588.51
			&42.12 \\
			
			\multicolumn{1}{ c }{\textsc{MIPplanet}}
			&1535.05
			& 
			&16.71
			
			&2239.23
			& 
			&42.76

			&2241.74
			& 
			&45.99 \\
			
			\multicolumn{1}{ c }{\textsc{Supergradient}}
			&155.12
			&2350.02
			&0.47
			
			&258.80
			&5304.62
			&0.00
			
			&1369.20
			&14574.71
			&23.77 \\
			
			\multicolumn{1}{ c }{\textsc{GNN}}
			& \B 131.86
			&1809.59
			&0.47
			
			& \B 217.70
			& 4174.40
			& 0.00
			
			& \B 1312.24
			& 13046.03
			& \B 23.26 \\
	
			\bottomrule
			
		\end{tabular}
	\end{adjustbox}
	\caption{\small We compare average (mean) solving time, average number of subdomains solved, and the percentage of properties solved for easy, medium, and hard properties on the base model. The best performing method for each subcategory is highlighted in bold. (Note that by definition Gurobi BaBSR doesn't time out on easy and med experiments)}.
	\label{table:easy_med_hard}
\end{table*}
